SpatialSplat: Efficient Semantic 3D from Sparse Unposed Images

A major breakthrough in 3D reconstruction is the feedforward paradigm to generate pixel-wise 3D points or Gaussian primitives from sparse, unposed images. To further incorporate semantics while avoiding the significant memory and storage costs of high-dimensional semantic features, existing methods extend this paradigm by associating each primitive with a compressed semantic feature vector. However, these methods have two major limitations: (a) the naively compressed feature compromises expressiveness, affecting the model's ability to capture fine-grained semantics, and (b) the pixel-wise primitive prediction introduces redundancy in overlapping areas, causing unnecessary memory overhead. To this end, we introduce \textbf{SpatialSplat}, a feedforward framework that produces redundancy-aware Gaussians and capitalizes on a dual-field semantic representation. Particularly, with the insight that primitives within the same instance exhibit high semantic consistency, we decompose the semantic representation into a coarse feature field that encodes uncompressed semantics with minimal primitives, and a fine-grained yet low-dimensional feature field that captures detailed inter-instance relationships. Moreover, we propose a selective Gaussian mechanism, which retains only essential Gaussians in the scene, effectively eliminating redundant primitives. Our proposed Spatialsplat learns accurate semantic information and detailed instances prior with more compact 3D Gaussians, making semantic 3D reconstruction more applicable. We conduct extensive experiments to evaluate our method, demonstrating a remarkable 60\% reduction in scene representation parameters while achieving superior performance over state-of-the-art methods. The code is available at https://github.com/shengyuuu/SpatialSplat.git

==> sec/tmp.tex <==
\section{intro}

Reconstructing and understanding 3D scenes from 2D data aims to extract geometric and semantic information from cost-effective sensors to overcome 3D data scarcity~\cite{reconstruction_survey}.
This task has broad applications in robotics navigation and manipulations~\cite{F3RM,GEFF}, digital twins~\cite{ScanNeRF}, and virtual/augmented reality (VR/AR)~\cite{AR,VR}.
Recent advances in 3D reconstruction and scene understanding have introduced promising representations, particularly 3D Gaussian Splatting (3DGS)\cite{3dgs}, which enables high-quality dense 3D reconstruction and photorealistic novel view synthesis.
However, 3DGS typically requires per-scene optimization, limiting its ability to generalize across multiple scenes.

As the number of input views increases, this redundancy becomes more pronounced, leading to substantial storage consumption.
Although FreeSplat~\cite{free-spalt} attempts to address this issue by projecting primitives onto a plane and identifying overlaps, its effectiveness is constrained when dealing with unposed images.

to compensate for the information loss introduced by compressed features, these methods still require relatively high-dimensional feature representations (e.g., 64-128)~\cite{lsm,Feature3dgs}, leading to suboptimal performance and escalating storage costs as the number of primitives increases.
Second,  we observe that existing feed-forward 3D Gaussian Splatting introducing 

unlike size-agnostic point clouds that rely on dense overlaps for detail capture, Gaussian primitives inherently encode regional textures~\cite{3dgs}.
This fundamental difference introduces significant redundancy in overlapping regions for existing feed-forward 3D Gaussian Splatting methods.

existing approaches~\cite{lsm,Feature3dgs,langsplat} mitigate the high storage/compute demands primitive-semantic learning by employing compressed features for each primitive. 
However, to compensate for the information loss introduced by compression, these methods still require relatively high-dimensional feature representations (e.g., 64-128)~\cite{Feature3dgs}, leading to suboptimal performance and escalating storage costs as the number of primitives increases.
Further more, we observe that existing feed-forward 3D Gaussian Splatting introducing 
Second, unlike size-agnostic point clouds that rely on dense overlaps for detail capture, Gaussian primitives inherently encode regional textures~\cite{3dgs}.
This fundamental difference introduces significant redundancy in overlapping regions for existing feed-forward 3D Gaussian Splatting methods.




Previous methods in this domain have introduced more powerful scene representations, such as Neural Radiance Field (NeRF)~\cite{NERF} and 3D Gaussian Splatting (3DGS)~\cite{3dgs}, enabling high-quality dense 3D reconstruction and photorealistic novel view synthesis. 
Subsequent innovations integrate vision-language models~\cite{CLIP} with these representations to extend radiance field to semantic feature fields~\cite{Feature-platting,Feature3dgs,langsplat}, thus enabling open-vocabulary 3D segmentation.
However, these approaches require time-consuming per-scene optimization and rely on precise camera poses, typically obtained via structure-from-motion (SfM)~\cite{colmap}, which has been shown to fail in textureless regions, limiting their applicability.
To further reduce time and alleviate the constraints of reconstruction, recent advancements have shifted towards end-to-end approaches, utilizing feed-forward networks to directly recover 3D scenes from posed~\cite{mvsplat,pixel-splat,free-spalt} or unposed~\cite{ye2024noposplat,smart2024splatt3r,instant-splat, wang2024dust3r, leroy2024mast3r} images.
A very recent method, Large Spatial Model (LSM)~\cite{lsm}, takes a step further by enabling 3D reconstruction and understanding from unposed images in a feed-forward Gaussian Splatting approach.
% \xnote{begin comment 1.}However, these approaches require time-consuming per-scene optimization and rely on precise camera poses, typically obtained via structure-from-motion (SfM), which has been shown to fail in textureless regions, limiting their applicability.
% Recent advances~\cite{mvsplat,pixel-splat,free-spalt} have shifted toward end-to-end approaches, leveraging feed-forward networks to directly recover 3D scenes from images.
% The DUSt3R series~\cite{wang2024dust3r,leroy2024mast3r} enables direct 3D pointmap prediction from unposed images, significantly simplifying the reconstruction process. 
% Building on this, recent methods~\cite{ye2024noposplat,smart2024splatt3r,instant-splat} have leveraged 3D pointmaps to predict pixelwise Gaussians by using them as Gaussian centers. \xnote{end comment 1.}
% Large Spatial Model (LSM)~\cite{lsm} extends this idea by enhancing each Gaussian with semantic features to construct a fine-grained semantic feature field, making it the first approach to achieve 3D scene reconstruction and understanding without relying on camera extrinsics.
% First, existing methods often overlook semantic consistency within instance and learning primitive-level semantics by employing compressed semantic features for each Gaussian primitive to reduce memory/storage demands  casued by the high dimension of semantic features.
% This compromise leads to suboptimal performance due to information loss during compression and growing storage costs as primitive counts increase.

Despite notable progress, critical challenges still persist. 
% First, existing methods often overlook semantic consistency within instance and learning primitive-level semantics by employing compressed semantic features for each Gaussian primitive to reduce memory/storage demands  casued by the high dimension of semantic features.
% This compromise leads to suboptimal performance due to information loss during compression and growing storage costs as primitive counts increase.
First, existing approaches~\cite{lsm,Feature3dgs,langsplat} mitigate the high storage/compute demands primitive-semantic learning by employing compressed features for each primitive. 
However, to compensate for the information loss introduced by compression, these methods still require relatively high-dimensional feature representations (e.g., 64-128)~\cite{Feature3dgs}, leading to suboptimal performance and escalating storage costs as the number of primitives increases.
Further more, we observe that existing feed-forward 3D Gaussian Splatting introducing 
Second, unlike size-agnostic point clouds that rely on dense overlaps for detail capture, Gaussian primitives inherently encode regional textures~\cite{3dgs}.
This fundamental difference introduces significant redundancy in overlapping regions for existing feed-forward 3D Gaussian Splatting methods.
% , as they depend on pixelwise Gaussian predictions based on binocular reconstruction—such as DUSt3r~\cite{wang2024dust3r}, which often requires overlapping input images to enhance performance.
As the number of input views increases, this redundancy becomes more pronounced, leading to substantial storage consumption.
Although FreeSplat~\cite{free-spalt} attempts to address this issue by projecting primitives onto a plane and identifying overlaps, its effectiveness is constrained when dealing with unposed images.
% However, naively assigning a high dimensional semantic feature (512 or more) to each 
% primitive results in significant storage and memory overhead.
% LSM~\cite{lsm} and other methods~\cite{GSemSplat,Feature3dgs,langsplat} have attempted to address this issue by compressing semantic features into lower dimensions and  recover them with an additional decoder.
% While this approach has yielded promising results, it introduces lossy feature compression, which degrades segmentation performance~\cite{Feature-platting}, ultimately leading to suboptimal results.
% Through an in-depth analysis, we argue that learning semantic features at the instance level, rather than the primitive level, is more efficient.
% As shown in Fig~\ref{first-fig}, semantic features within the same instance are highly similar or even identical, meaning fine-grained semantic feature maps can be reconstructed using coarse feature maps and corresponding instance segmentation results, as demonstrated in~\cite{Feature-platting} 
% Additionally, unlike point clouds, which lack size properties and rely on dense overlap to capture fine details, Gaussians inherently represent regional textures~\cite{3dgs}.
% This characteristic introduces significant redundancy in overlapping regions for existing feed-forward 3D Gaussian Splatting methods, as they depend on pixel-wise Gaussian predictions based on binocular reconstruction—such as DUSt3r~\cite{wang2024dust3r}, which often requires overlapping input images to enhance performance.\xnote{discuss.}

% Thanks to its compact design, SpatialSplat can efficiently incorporate more views or higher-resolution inputs, extending 3D scene understanding to larger environments and enhancing scalability.

% % reconstruction : pixelwise gaussian 
% % semantic : primitive learning -> compression feature -> information loss
% Recent breakthroughs in scene reconstruction have introduced promising representations, `, 3D Gaussian Splatting (3DGS)~\cite{3dgs}, which enables high-quality dense 3D reconstruction and photorealistic novel view synthesis. 
% The method typically requires per-scene optimization that limits the ability to share a single model across multiple scenes.

% Subsequent works\cite{pixel-splat, mvsplat, free-spalt} address this through feed-forward networks enabling cross-scene generalization and accelerated reconstruction.
% Further advancements~\cite{smart2024splatt3r,ye2024noposplat} extend generalizable 3DGS to unposed images based on DUSt3R~\cite{wang2024dust3r}, eliminating the need for explicit camera poses.
% Parallel efforts~\cite{Feature3dgs,langsplat,Feature-platting} have sought to enrich scene representations with semantic understanding by integrating vision-language models~\cite{CLIP,lseg} to construct a dense semantic feature field.
% The state-of-the-art (SOTA) method, Large Spatial Model (LSM)~\cite{lsm}, takes a step further by combining generalized 3D reconstruction with language models, allowing for faster and more flexible scene understanding.
% However, incorporating high-dimensional (512 or more) language features introduces substantial computational and storage overhead, which researchers~\cite{lsm,Feature3dgs} have attempted to mitigate by compressing these features into lower-dimensional representations (e.g., 64-128).

% Despite notable progress, critical challenges remain. 
% First, compressing semantic features introduces irreversible information loss~\cite{Feature3dgs}, leading to suboptimal performance, while still incurring significant storage costs as the number of primitives grows. 
% Second,  we observe existing feed-forward 3DGS methods tend to generate redundant Gaussian primitives in overlapping regions (Fig.\ref{fig:first-fig}), leading to significant storage overhead with minimal accuracy gains. 
% This redundancy becomes more pronounced as the number of input views increases. 
% While FreeSplat~\cite{free-spalt} attempts to address this issue by projecting primitives onto a plane and identifying overlaps, its effectiveness is limited when dealing with unposed images.

% To address these limitations, we propose SpatialSplat, a feed-forward network generating compact yet expressive semantic 3D representations from unposed images. 
% Specifically, SpatialSplat introduces a dual-field architecture that decomposes the dense semantic feature field into two components: a coarse feature field encoding uncompressed instance-level semantics through minimal Gaussians, and a low-dimensional fine-grained feature field capturing inter-instance relationships. 
% Our key insight is the observation that the Gaussian primitives within the same instance exhibit strong semantic consistency. 
% By preserving uncompressed semantics and capturing instance information with clearer boundaries, our method achieves superior segmentation performance with reduced representation parameters.
% Additionally, we introduce a Selective Gaussian Mechanism (SGM) to eliminate redundancy in overlapping areas caused by pixelwise representations, accompanied by a novel loss function that jointly optimizes Gaussian sparsity and scene fidelity.
% Extensive experiments demonstrate that our method achieves state-of-the-art performance while using only 40$\%$ of the scene representation parameters required by the baseline, all without any 3D supervision. 
